Active Finite Reward Automaton Inference and Reinforcement Learning Using Queries and Counterexamples

Despite the fact that deep reinforcement learning (RL) has surpassed human-level performances in various tasks, it still has several fundamental challenges. First, most RL methods require intensive data from the exploration of the environment to achieve satisfactory performance. Second, the use of neural networks in RL renders it hard to interpret the internals of the system in a way that humans can understand. To address these two challenges, we propose a framework that enables an RL agent to reason over its exploration process and distill high-level knowledge for effectively guiding its future explorations. Specifically, we propose a novel RL algorithm that learns high-level knowledge in the form of a finite reward automaton by using the L* learning algorithm. We prove that in episodic RL, a finite reward automaton can express any non-Markovian bounded reward functions with finitely many reward values and approximate any non-Markovian bounded reward function (with infinitely many reward values) with arbitrary precision. We also provide a lower bound for the episode length such that the proposed RL approach almost surely converges to an optimal policy in the limit. We test this approach on two RL environments with non-Markovian reward functions, choosing a variety of tasks with increasing complexity for each environment. We compare our algorithm with the state-of-the-art RL algorithms for non-Markovian reward functions, such as Joint Inference of Reward machines and Policies for RL (JIRP), Learning Reward Machine (LRM), and Proximal Policy Optimization (PPO2). Our results show that our algorithm converges to an optimal policy faster than other baseline methods.

==> Active automata learning RL final2/macros.tex <==
% !TEX root = main.tex


\newtcbox{\remind}{%
  enhanced jigsaw,nobeforeafter,size=fbox,sharp corners,
  shrink tight,
  extrude by=3pt,
  tcbox raise base,
  borderline={0.5pt}{-1pt}{red,opacity=0.75},
  opacityframe=0.75,
  opacityback=0.5,
}

% math operators
\newcommand{\argmin}{\mathrm{arg}\min}  
\newcommand{\argsup}{\mathrm{arg}\sup}
\newcommand{\arginf}{\mathrm{arg}\inf}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

\newcommand{\setOfQFunctions}{Q}
\newcommand{\setOfQFunctionsNew}{Q_{\textrm{new}}}            

\newcommand{\set}[1]{\{ #1 \}}
\newcommand{\reals}{\mathbb{R}}

% tabs
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}

% Case Studies

\newcommand{\methodA}{JIRP}
\newcommand{\methodB}{QAS}
\newcommand{\methodC}{HRL} 

% \newcommand{\Traffic}{Autonomous Vehicle Scenario}
% \newcommand{\traffic}{autonomous vehicle scenario}
% \newcommand{\TrafficA}{Task 1.1}
% \newcommand{\trafficA}{task 1.1}
% \newcommand{\TrafficB}{Task 1.2}
% \newcommand{\trafficB}{task 1.2}
% \newcommand{\TrafficC}{Task 1.3}
% \newcommand{\trafficC}{task 1.3}
% \newcommand{\TrafficD}{Task 1.4}
% \newcommand{\trafficD}{task 1.4}

\newcommand{\Qlearning}{Q-learning}
\newcommand{\HRL}{HRL}

\newcommand{\Office}{Office World Scenario}
\newcommand{\office}{office world scenario}
\newcommand{\OfficeA}{Task 1}
\newcommand{\officeA}{task 1}
\newcommand{\OfficeB}{Task 2}
\newcommand{\officeB}{task 2}
\newcommand{\OfficeC}{Task 3}
\newcommand{\officeC}{task 3} 
\newcommand{\OfficeD}{Task 4}
\newcommand{\officeD}{task 4}

\newcommand{\Craft}{Minecraft World Scenario}
\newcommand{\craft}{Minecraft world scenario}
\newcommand{\CraftA}{Task 3.1}
\newcommand{\craftA}{task 3.1}
\newcommand{\CraftB}{Task 3.2}
\newcommand{\craftB}{task 3.2}
\newcommand{\CraftC}{Task 3.3}
\newcommand{\craftC}{task 3.3}
\newcommand{\CraftD}{Task 3.4}
\newcommand{\craftD}{task 3.4}


% RL 
\newcommand{\policy}{\pi}
\newcommand{\qValue}{q}
\newcommand{\qValueNew}{q_{\textrm{new}}}
\newcommand{\Reward}{r}
\newcommand{\maxLengthEpisode}{m}

% comments
\newcommand{\IG}[1]{{\color{red} IG: #1}}
\newcommand{\ZX}[1]{{\color{blue} ZX: #1}}
\newcommand{\BW}[1]{{\color{green} BW: #1}}
\newcommand{\DN}[1]{{\color{orange!90!black} DN: #1}}
\newcommand{\RM}[1]{{\color{pink} RM: #1}}
\newcommand{\UT}[1]{{\color{brown} UT: #1}}

\newcommand{\implement}{encode}
\newcommand{\implementing}{encoding}


% QRM
\newcommand{\algoName}{JIRP} 
\newcommand{\newAlgoName}{AFRAI-RL} 
\newcommand{\algoOptName}{JIRP with the algorithmic optimizations}
\newcommand{\correctingSet}{C}
\newcommand{\allExperiences}{\Omega}
\newcommand{\hypothesisRM}{\mathcal H}
\newcommand{\hypothesisRMnew}{\mathcal H_{\textrm{new}}}
\newcommand{\counterexamples}{X}
\newcommand{\newCounterexamples}{X_{\textrm{new}}}

%\newcommand{\Trace}{\tau}
%\newcommand{\RewardTrace}{\eta}


\newcommand{\init}{I}


% DFA
\newcommand{\dfaStates}{V}
\newcommand{\dfaState}{v}
\newcommand{\dfaInit}{\dfaState_\init}
\newcommand{\dfaTransition}{\delta}
\newcommand{\dfaInputAlphabet}{\Sigma}
\newcommand{\dfaWord}{\omega}
\newcommand{\dfaFinalStates}{F}
\newcommand{\dfa}{\mathfrak A}
\newcommand{\word}{\omega}
\newcommand{\dfaSymbol}{\ensuremath{b}}


% MDP
\newcommand{\mdp}{\mathcal{M}} 
\newcommand{\mdpStates}{X}
\newcommand{\mdpState}{x}
\newcommand{\mdpInit}{\mdpState_{init}}
\newcommand{\mdpActions}{A}
\newcommand{\mdpAction}{a}
\newcommand{\mdpProb}{p}
\newcommand{\mdpRewardFunction}{R}
\newcommand{\mdpDiscount}{\gamma}
\newcommand{\mdpTrajectory}{\zeta}
\newcommand{\mdpLabel}{\ell}
\newcommand{\mdpRewards}{r}
\newcommand{\trajectory}[1]{\ensuremath{\mdpState_0 \mdpAction_0\ldots \mdpState_{#1} \mdpAction_{#1} \mdpState_{#1 + 1}}}

% NMRDP
\newcommand{\nmrdpRewards}{\mdpRewards_N}

% reward machines
\newcommand{\rmLabels}{\mathcal P}
\newcommand{\rmLabelingFunction}{L}
\newcommand{\rmRewardFunction}{\rho}
\newcommand{\rmInputAlphabet}{2^\rmLabels}
\newcommand{\rmOutputAlphabet}{\mathcal{R}}


% reward machines
\newcommand{\machine}{\mathcal A}
\newcommand{\mealyStates}{W}

\newcommand{\mealyState}{w}
\newcommand{\mealyInput}{u}        
\newcommand{\mealyInputAlphabet}{\ensuremath{{2^\mathcal{P}}}}
\newcommand{\mealyInit}{{\mealyState_{init}}}
\newcommand{\mealyInitHat}{{\hat{\mealyState}_{init}}}
\newcommand{\mealyOutputAlphabet}{\ensuremath{\mathcal{R}}}
\newcommand{\mealyOutput}{\eta}
\newcommand{\mealyTransition}{\delta}
\newcommand{\inputTrace}{\lambda}
\newcommand{\outputTrace}{\rho}


\newcommand{\mealyOutputNew}{\mealyOutput_{\textrm{new}}}
\newcommand{\mealyTransitionNew}{\mealyTransition_{\textrm{new}}}
\newcommand{\mealyStatesNew}{\mealyStates_{\textrm{new}}}
\newcommand{\mealyStateNew}{\mealyState_{\textrm{new}}}
\newcommand{\mealyInitNew}{\mealyInit_{\textrm{new}}}

% automata learning
\newcommand{\sample}{\mathcal{S}}
\newcommand{\pClass}{\mathcal{S}^{+}}
\newcommand{\nClass}{\mathcal{S}^{-}}
\newcommand{\RPNIMealy}{RPNI-RM}

